MOJAVE. X. Parsec-Scale Jet Orientation Variations and Superluminal Motion in AGN

We describe the parsec-scale kinematics of 200 AGN jets based on 15 GHz VLBA data obtained between 1994 Aug 31 and 2011 May 1. We present new VLBA 15 GHz images of these and 59 additional AGN from the MOJAVE and 2 cm Survey programs. Nearly all of the 60 most heavily observed jets show significant changes in their innermost position angle over a 12 to 16 year interval, ranging from 10 deg to 150 deg on the sky, corresponding to intrinsic variations of ~0.5 deg to ~2 deg. The BL Lac jets show smaller variations than quasars. Roughly half of the heavily observed jets show systematic position angle trends with time, and 20 show indications of oscillatory behavior. The time spans of the data sets are too short compared to the fitted periods (5 to 12 y), however, to reliably establish periodicity. The rapid changes and large jumps in position angle seen in many cases suggest that the superluminal AGN jet features occupy only a portion of the entire jet cross section, and may be energized portions of thin instability structures within the jet. We have derived vector proper motions for 887 moving features in 200 jets having at least five VLBA epochs. For 557 well-sampled features, there are sufficient data to additionally study possible accelerations. We find that the moving features are generally non-ballistic, with 70% of the well-sampled features showing either significant accelerations or non-radial motions. Inward motions are rare (2% of all features), are slow (<0.1 mas per y), are more prevalent in BL Lac jets, and are typically found within 1 mas of the unresolved core feature. There is a general trend of increasing apparent speed with distance down the jet for both radio galaxies and BL Lac objects. In most jets, the speeds of the features cluster around a characteristic value, yet there is a considerable dispersion in the distribution. (abridged)

==> gentable.tex <==
\begin{deluxetable}{llllccc} 
\tablecolumns{7} 
\tabletypesize{\scriptsize} 
\tablewidth{0pt}  
\tablecaption{\label{gentable} General Properties of AGNs in the Combined Samples}  
\tablehead{\colhead{B1950} & \colhead {Alias} &\colhead{2FGL Assoc.} &  
\colhead{z} &  \colhead{Ref.} & \colhead{Opt.}& \colhead{Sample} \\ 
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & 
 \colhead{(6)} & \colhead{(7)}} 
\startdata 
0003+380 & S4 0003+38& J0006.1+3821 & 0.229& \cite{1994AAS..103..349S} & Q& L \\ 
0003$-$066 & NRAO 005&\n & 0.3467& \cite{2005PASA...22..277J} & B& R \\ 
0007+106 & III Zw 2&\n & 0.0893& \cite{1970ApJ...160..405S} & G& R,L \\ 
0010+405 & 4C +40.01&\n & 0.256& \cite{1992ApJS...81....1T} & Q& L \\ 
0015$-$054 & PMN J0017$-$0512& J0017.6$-$0510 & 0.226& \cite{2012ApJ...748...49S} & Q& G,L \\ 
0016+731 & S5 0016+73&\n & 1.781& \cite{1986AJ.....91..494L} & Q& R \\ 
0048$-$097 & PKS 0048$-$09& J0050.6$-$0929 & 0.635& \cite{2012AA...543A.116L} & B& G,R \\ 
0055+300 & NGC 315&\n & 0.0165& \cite{1999ApJS..121..287H} & G& L \\ 
0059+581 & TXS 0059+581& J0102.7+5827 & 0.644& \cite{2005ApJ...626...95S} & Q& R \\ 
0106+013 & 4C +01.02& J0108.6+0135 & 2.099& \cite{1995AJ....109.1498H} & Q& G,R \\ 
0109+224 & S2 0109+22& J0112.1+2245 & 0.265& \cite{2012ApJ...748...49S} & B& G,R \\ 
0109+351 & B2 0109+35&\n & 0.450& \cite{1996MNRAS.282.1274H} & Q& R \\ 
0110+318 & 4C +31.03& J0112.8+3208 & 0.603& \cite{1976ApJS...31..143W} & Q& G \\ 
0111+021 & UGC 00773&\n & 0.047& \cite{1976ApJS...31..143W} & B& L \\ 
0116$-$219 & OC -228& J0118.8$-$2142 & 1.165& \cite{1983MNRAS.205..793W} & Q& G \\ 
0118$-$272 & OC -230.4& J0120.4$-$2700 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0119+115 & PKS 0119+11&\n & 0.570& \cite{1994AAS..105..211S} & Q& R \\ 
0122$-$003 & UM 321&\n & 1.0765& \cite{2002AJ....123..567S} & Q& R \\ 
0130$-$171 & OC -150& J0132.8$-$1654 & 1.020& \cite{1983MNRAS.205..793W} & Q& G,R \\ 
0133+388\tablenotemark{a} & B3 0133+388& J0136.5+3905 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0133+476 & DA 55& J0136.9+4751 & 0.859& \cite{1986AJ.....91..494L} & Q& G,R \\ 
0142$-$278 & OC -270& J0145.1$-$2732 & 1.148& \cite{1999ApJS..122...29B} & Q& G \\ 
0202+149 & 4C +15.05& J0205.0+1514 & 0.405& \cite{1998AJ....115.1253P} & Q& R \\ 
0202+319 & B2 0202+31& J0205.4+3211 & 1.466& \cite{1970ApJ...160L..33B} & Q& R \\ 
0202$-$172 & PKS 0202$-$17& J0205.3$-$1657 & 1.739& \cite{2009MNRAS.399..683J} & Q& R \\ 
0208+106 & MG1 J021114+1051& J0211.2+1050 & 0.20& \cite{2010ApJ...712...14M} & B& R,L \\ 
0212+735 & S5 0212+73& J0217.7+7353 & 2.367& \cite{1986AJ.....91..494L} & Q& R \\ 
0215+015 & OD 026& J0217.9+0143 & 1.715& \cite{1988AA...192....1B} & Q& G,R \\ 
0219+428\tablenotemark{a} & 3C 66A& J0222.6+4302 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0224+671 & 4C +67.05&\n & 0.523& \cite{2005ApJ...626...95S} & Q& R \\ 
0229+131 & 4C +13.14&\n & 2.059& \cite{1994ApJ...436..678O} & Q& R \\ 
0234+285 & 4C +28.07& J0237.8+2846 & 1.206& \cite{2012ApJ...748...49S} & Q& G,R \\ 
0235+164 & AO 0235+164& J0238.7+1637 & 0.940& \cite{1987ApJ...318..577C} & Q& G,R \\ 
0238$-$084 & NGC 1052&\n & 0.005037& \cite{2005MNRAS.356.1440D} & G& R,L \\ 
0241+622 & 7C 0241+6215&\n & 0.045& \cite{2003ApJS..145..199M} & Q& R,L \\ 
0250$-$225 & OD -283& J0252.7$-$2218 & 1.419& \cite{2012ApJ...748...49S} & Q& G \\ 
0300+470 & 4C +47.08& J0303.5+4713 & \n& \cite{2013ApJ...764..135S} & B& R \\ 
0301$-$243\tablenotemark{a} & PKS 0301$-$243& J0303.4$-$2407 & 0.266& \cite{2012arXiv1208.1785P} & B& G,L \\ 
0305+039 & 3C 78&\n & 0.029& \cite{1998AA...333...48P} & G& L \\ 
0309+411 & NRAO 128&\n & 0.136& \cite{1996MNRAS.281..425M} & G& L \\ 
0313+088 & BZB J0316+0904& J0316.1+0904 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0316+413\tablenotemark{a} & 3C 84& J0319.8+4130 & 0.0176& \cite{1992ApJS...83...29S} & G& G,R,L \\ 
0333+321 & NRAO 140& J0337.0+3200c & 1.259& \cite{1991ApJ...382..433S} & Q& R \\ 
0336$-$019 & CTA 26& J0339.4$-$0144 & 0.852& \cite{1978ApJS...36..317W} & Q& R \\ 
0347$-$211 & OE -280& J0350.0$-$2104 & 2.944& \cite{2001AA...379..393E} & Q& G \\ 
0355+508 & NRAO 150&\n & 1.520& \cite{2007AA...476L..17A} & Q& R \\ 
0400+258 & CTD 026&\n & 2.109& \cite{1977ApJ...217..358S} & Q& R \\ 
0403$-$132 & PKS 0403$-$13& J0405.8$-$1309 & 0.571& \cite{1996ApJS..104...37M} & Q& R \\ 
0415+379 & 3C 111&\n & 0.0491& \cite{2004ApJS..150..181E} & G& R,L \\ 
0420$-$014 & PKS 0420$-$01& J0423.2$-$0120 & 0.9161& \cite{2009MNRAS.399..683J} & Q& G,R \\ 
0422+004 & PKS 0422+00& J0424.7+0034 & 0.268& \cite{2013ApJ...764..135S} & B& R \\ 
0430+052 & 3C 120&\n & 0.033& \cite{1988PASP..100.1423M} & G& R,L \\ 
0430+289 & BZB J0433+2905& J0433.5+2905 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0440$-$003 & NRAO 190& J0442.7$-$0017 & 0.845& \cite{2012ApJ...748...49S} & Q& G,R \\ 
0446+112 & PKS 0446+11& J0448.9+1121 & 2.153& \cite{2012ApJ...748...49S} & Q& R \\ 
0451$-$282 & OF -285& J0453.1$-$2807 & 2.559& \cite{1983MNRAS.205..793W} & Q& G,R \\ 
0454$-$234 & PKS 0454$-$234& J0457.0$-$2325 & 1.003& \cite{1989AAS...80..103S} & Q& G,R \\ 
0458$-$020 & S3 0458$-$02& J0501.2$-$0155 & 2.286& \cite{1974ApJ...190..509S} & Q& R \\ 
0502+675\tablenotemark{a} & 1ES 0502+675& J0508.0+6737 & 0.340& \cite{2013ApJ...764..135S} & B& G,L \\ 
0506+056 & TXS 0506+056& J0509.4+0542 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0528+134 & PKS 0528+134& J0530.8+1333 & 2.070& \cite{1993ApJ...409..134H} & Q& G,R \\ 
0529+075 & OG 050& J0532.7+0733 & 1.254& \cite{2005ApJ...626...95S} & Q& G,R \\ 
0529+483 & TXS 0529+483& J0533.0+4823 & 1.160& \cite{2012ApJ...748...49S} & Q& R \\ 
0539$-$057 & PKS 0539$-$057&\n & 0.838& \cite{2012ApJ...748...49S} & Q& R \\ 
0552+398 & DA 193&\n & 2.363& \cite{1999ApJ...514...40M} & Q& R \\ 
0605$-$085 & OC -010& J0608.0$-$0836 & 0.870& \cite{2012ApJ...748...49S} & Q& R \\ 
0605$-$153 & PMN J0608$-$1520& J0608.0$-$1521 & 1.094& \cite{2012ApJ...748...49S} & Q& G \\ 
0607$-$157 & PKS 0607$-$15&\n & 0.3226& \cite{2009MNRAS.399..683J} & Q& R \\ 
0609+413 & B3 0609+413& J0612.8+4122 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
0628$-$240 & TXS 0628$-$240& J0630.9$-$2406 & 1.60& \cite{2012AA...538A..26R} & B& G \\ 
0642+449 & OH 471&\n & 3.396& \cite{1994ApJ...436..678O} & Q& R \\ 
0648$-$165 & PKS 0648$-$16& J0650.4$-$1632 & \n& \n & U& R \\ 
0650+453 & B3 0650+453& J0654.2+4514 & 0.928& \cite{2012ApJ...748...49S} & Q& G \\ 
0650+507 & GB6 J0654+5042& J0654.5+5043 & 1.253& \cite{2012ApJ...748...49S} & Q& G \\ 
0710+196 & WB92 0711+1940& J0714.0+1933 & 0.540& \cite{2012ApJ...748...49S} & Q& G \\ 
0716+332 & B2 0716+33& J0719.3+3306 & 0.779& \cite{2000ApJS..126..133W} & Q& G \\ 
0716+714\tablenotemark{a} & S5 0716+71& J0721.9+7120 & \n& \cite{2008AA...487L..29N} & B& G,R \\ 
0723$-$008 & PKS 0723$-$008& J0726.0$-$0053 & 0.127& \cite{1976ApJS...31..143W} & B& R \\ 
0727$-$115 & PKS 0727$-$11& J0730.2$-$1141 & 1.591& \cite{2002AJ....124..662Z} & Q& R \\ 
0730+504 & TXS 0730+504& J0733.9+5023 & 0.720& \cite{1997MNRAS.290..380H} & Q& R \\ 
0735+178 & OI 158& J0738.0+1742 & 0.450& \cite{2012arXiv1209.4755N} & B& G,R \\ 
0736+017 & OI 061& J0739.2+0138 & 0.1894& \cite{2009ApJS..184..398H} & Q& G,R \\ 
0738+313 & OI 363&\n & 0.631& \cite{2004AJ....128..502A} & Q& R \\ 
0742+103 & PKS B0742+103&\n & 2.624& \cite{2003MNRAS.346.1021B} & Q& R \\ 
0743$-$006 & OI -072&\n & 0.996& \cite{1989AAS...80..103S} & Q& R \\ 
0745+241 & PKS 0745+241&\n & 0.4092& \cite{2004AJ....128..502A} & Q& R \\ 
0748+126 & OI 280& J0750.6+1230 & 0.889& \cite{1979ApJ...232..400P} & Q& R \\ 
0754+100 & PKS 0754+100& J0757.1+0957 & 0.266& \cite{2003AA...412..651C} & B& R \\ 
0804+499 & BZQ J0808+4950&\n & 1.436& \cite{2006ApJS..162...38A} & Q& R \\ 
0805$-$077 & PKS 0805$-$07& J0808.2$-$0750 & 1.837& \cite{1988ApJ...327..561W} & Q& G,R \\ 
0808+019 & OJ 014& J0811.4+0149 & 1.148& \cite{2005AJ....129..559S} & B& R \\ 
0814+425 & OJ 425& J0818.2+4223 & \n& \cite{2013ApJ...764..135S} & B& G,R \\ 
0821+394 & 4C +39.23& J0824.7+3914 & 1.216& \cite{2005AJ....130..367S} & Q& R \\ 
0823+033 & PKS 0823+033& J0825.9+0308 & 0.505& \cite{2013ApJ...764..135S} & B& R \\ 
0827+243 & OJ 248& J0830.5+2407 & 0.942& \cite{2012ApJ...748...49S} & Q& R \\ 
0829+046 & OJ 049& J0831.9+0429 & 0.174& \cite{2005AJ....129.1755A} & B& R,L \\ 
0834$-$201 & PKS 0834$-$20&\n & 2.752& \cite{1983AA...117...60F} & Q& R \\ 
0836+710 & 4C +71.07& J0841.6+7052 & 2.218& \cite{1993AAS..100..395S} & Q& R \\ 
0838+133 & 3C 207& J0840.7+1310 & 0.680& \cite{2012ApJ...748...49S} & Q& R \\ 
0847$-$120 & BZQ J0850$-$1213& J0850.2$-$1212 & 0.566& \cite{1997IAUC.6639....2H} & Q& R \\ 
0851+202 & OJ 287& J0854.8+2005 & 0.306& \cite{1989AAS...80..103S} & B& G,R \\ 
0859$-$140 & PKS B0859$-$140&\n & 1.339& \cite{1997MNRAS.284...85D} & Q& R \\ 
0906+015 & 4C +01.24& J0909.1+0121 & 1.026& \cite{2012ApJ...748...49S} & Q& G,R \\ 
0917+449 & S4 0917+44& J0920.9+4441 & 2.189& \cite{2004AJ....128..502A} & Q& G,R \\ 
0917+624 & OK 630& J0921.9+6216 & 1.453& \cite{2012ApJ...748...49S} & Q& R \\ 
0923+392 & 4C +39.25&\n & 0.695& \cite{2004AJ....128..502A} & Q& R \\ 
0945+408 & 4C +40.24& J0948.8+4040 & 1.249& \cite{2004AJ....128..502A} & Q& R \\ 
0946+006 & PMN J0948+0022& J0948.8+0020 & 0.585& \cite{2004AJ....128..502A} & N& G \\ 
0954+556 & 4C +55.17& J0957.7+5522 & 0.899& \cite{2012ApJ...748...49S} & Q& G \\ 
0954+658 & S4 0954+65& J0958.6+6533 & 0.367& \cite{2001AJ....122..565R} & B& R \\ 
0955+476 & OK 492& J0957.7+4735 & 1.882& \cite{2004AJ....128..502A} & Q& R \\ 
1009+249 & GB6 J1012+2439& J1012.6+2440 & 1.80& \cite{2012ApJ...748...49S} & Q& G \\ 
1011+496\tablenotemark{a} & 1ES 1011+496& J1015.1+4925 & 0.212& \cite{2007ApJ...667L..21A} & B& G,L \\ 
1013+054 & TXS 1013+054& J1016.0+0513 & 1.713& \cite{2004AJ....128..502A} & Q& G \\ 
1030+415 & S4 1030+41& J1033.2+4117 & 1.117& \cite{2007AJ....134..102S} & Q& R \\ 
1034+574 & GB6 J1037+5711& J1037.6+5712 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1034$-$293 & PKS 1034$-$293&\n & 0.312& \cite{1989AAS...80..103S} & Q& R \\ 
1036+054 & PKS 1036+054&\n & 0.473& \cite{2008ApJS..175...97H} & Q& R \\ 
1038+064 & 4C +06.41& J1040.7+0614 & 1.265& \cite{1991ApJ...382..433S} & Q& R \\ 
1045$-$188 & PKS 1045$-$18&\n & 0.595& \cite{1993AAS...97..483S} & Q& R \\ 
1055+018 & 4C +01.28& J1058.4+0133 & 0.888& \cite{2012ApJ...748...49S} & Q& G,R \\ 
1055+567 & 7C 1055+5644& J1058.6+5628 & 0.143& \cite{2004AJ....128..502A} & B& G,L \\ 
1101+384\tablenotemark{a} & Mrk 421& J1104.4+3812 & 0.0308& \cite{1975ApJ...198..261U} & B& G,L \\ 
1118$-$056 & PKS 1118$-$05& J1121.5$-$0554 & 1.297& \cite{1997MNRAS.284...85D} & Q& G \\ 
1124$-$186 & PKS 1124$-$186& J1126.6$-$1856 & 1.048& \cite{1997MNRAS.284...85D} & Q& R \\ 
1127$-$145 & PKS 1127$-$14& J1130.3$-$1448 & 1.184& \cite{1986MNRAS.218..331W} & Q& G,R \\ 
1128+385 & B2 1128+38&\n & 1.733& \cite{2007AJ....134..102S} & Q& R \\ 
1128$-$047 & PKS 1128$-$047&\n & 0.266& \cite{1997MNRAS.284...85D} & G& L \\ 
1150+497 & 4C +49.22& J1153.2+4935 & 0.3334& \cite{2007AJ....134..102S} & Q& R \\ 
1150+812 & S5 1150+81&\n & 1.250& \cite{1986AA...168...17E} & Q& R \\ 
1156+295 & 4C +29.45& J1159.5+2914 & 0.725& \cite{2012ApJ...748...49S} & Q& G,R \\ 
1213$-$172 & PKS 1213$-$17&\n & \n& \n & U& R \\ 
1215+303\tablenotemark{a} & ON 325& J1217.8+3006 & 0.130& \cite{2003ApJS..148..275A} & B& G,L \\ 
1218+304\tablenotemark{a} & B2 1218+30& J1221.3+3010 & 0.184& \cite{2013ApJ...764..135S} & B& G,L \\ 
1219+044 & 4C +04.42& J1222.4+0413 & 0.966& \cite{2012ApJ...748...49S} & Q& R \\ 
1219+285\tablenotemark{a} & W Comae& J1221.4+2814 & 0.103& \cite{2013ApJ...764..135S} & B& G \\ 
1222+216\tablenotemark{a} & 4C +21.35& J1224.9+2122 & 0.434& \cite{2009ApJS..182..543A} & Q& G,R \\ 
1226+023 & 3C 273& J1229.1+0202 & 0.1583& \cite{1992ApJS...83...29S} & Q& G,R \\ 
1228+126\tablenotemark{a} & M87& J1230.8+1224 & 0.00436& \cite{2000MNRAS.313..469S} & G& R,L \\ 
1236+049 & BZQ J1239+0443& J1239.5+0443 & 1.761& \cite{2012ApJ...748...49S} & Q& G \\ 
1244$-$255 & PKS 1244$-$255& J1246.7$-$2546 & 0.633& \cite{1976MNRAS.177P..77S} & Q& G \\ 
1246+586 & PG 1246+586& J1248.2+5820 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1253$-$055\tablenotemark{a} & 3C 279& J1256.1$-$0547 & 0.536& \cite{1996ApJS..104...37M} & Q& G,R \\ 
1300+248 & VIPS 0623 & J1303.1+2435 & 0.993& \cite{2007ApJ...667..673G} & B& G \\ 
1302$-$102 & PG 1302$-$102&\n & 0.278& \cite{1996ApJS..104...37M} & Q& L \\ 
1308+326 & OP 313& J1310.6+3222 & 0.997& \cite{2012ApJ...748...49S} & Q& G,R \\ 
1324+224 & B2 1324+22& J1326.8+2210 & 1.403& \cite{2012ApJ...748...49S} & Q& R \\ 
1329$-$049 & OP -050& J1332.0$-$0508 & 2.150& \cite{1990PASP..102.1235T} & Q& G,R \\ 
1329$-$126 & PMN J1332$-$1256& J1332.5$-$1255 & 1.492& \cite{2012ApJ...748...49S} & Q& G \\ 
1334$-$127 & PKS 1335$-$127& J1337.7$-$1257 & 0.539& \cite{1993AAS...97..483S} & Q& G,R \\ 
1341$-$171 & PMN J1344$-$1723& J1344.2$-$1723 & 2.506& \cite{2012ApJ...748...49S} & Q& G \\ 
1345+125 & 4C +12.50&\n & 0.121& \cite{1994ApJS...91..491G} & G& L \\ 
1406$-$076 & PKS B1406$-$076& J1408.8$-$0751 & 1.494& \cite{1979ApJ...232..400P} & Q& R \\ 
1413+135 & PKS B1413+135& J1416.0+1323 & 0.247& \cite{1992ApJ...400L..17S} & B& R \\ 
1417+385 & B3 1417+385& J1419.4+3820 & 1.831& \cite{2006ApJS..162...38A} & Q& R \\ 
1418+546 & OQ 530& J1420.2+5422 & 0.153& \cite{2013ApJ...764..135S} & B& L \\ 
1424+240\tablenotemark{a} & OQ 240& J1427.0+2347 & \n& \cite{2010ApJ...712...14M} & B& G,L \\ 
1435+638 & VIPS 0792&\n & 2.066& \cite{1999ApJ...514...40M} & Q& R \\ 
1458+718 & 3C 309.1&\n & 0.904& \cite{1997AJ....114.2254S} & Q& R \\ 
1502+106 & OR 103& J1504.3+1029 & 1.8385& \cite{2008ApJS..175..297A} & Q& G,R \\ 
1504$-$166 & PKS 1504$-$167&\n & 0.876& \cite{1978MNRAS.185..149H} & Q& R \\ 
1509+054 & PMN J1511+0518&\n & 0.084& \cite{2001ARep...45...79C} & G& L \\ 
1510$-$089\tablenotemark{a} & PKS 1510$-$08& J1512.8$-$0906 & 0.360& \cite{1990PASP..102.1235T} & Q& G,R \\ 
1514+004 & CGCG 021$-$063&\n & 0.052& \cite{2008ApJS..175...97H} & G& L \\ 
1514+197 & PKS 1514+197& J1516.9+1925 & \n& \cite{2013ApJ...764..135S} & B& R \\ 
1514$-$241\tablenotemark{a} & AP Librae& J1517.7$-$2421 & 0.049& \cite{2009MNRAS.399..683J} & B& G,R,L \\ 
1519$-$273 & PKS 1519$-$273& J1522.7$-$2731 & 1.297& \cite{2004AA...418..813H} & B& R \\ 
1520+319 & B2 1520+31& J1522.1+3144 & 1.484& \cite{2012ApJ...748...49S} & Q& G \\ 
1538+149 & 4C +14.60& J1540.4+1438 & 0.606& \cite{2013ApJ...764..135S} & B& R \\ 
1542+616 & GB6 J1542+6129& J1542.9+6129 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1546+027 & PKS 1546+027& J1549.5+0237 & 0.414& \cite{2004AJ....128..502A} & Q& R \\ 
1548+056 & 4C +05.64& J1550.7+0526 & 1.417& \cite{2012ApJ...748...49S} & Q& R \\ 
1551+130 & OR 186& J1553.5+1255 & 1.308& \cite{2009ApJS..182..543A} & Q& G \\ 
1553+113\tablenotemark{a} & PG 1553+113& J1555.7+1111 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1606+106 & 4C +10.45& J1608.5+1029 & 1.232& \cite{2012ApJ...748...49S} & Q& R \\ 
1611+343 & DA 406& J1613.4+3409 & 1.40& \cite{2012ApJ...748...49S} & Q& R \\ 
1622$-$253 & PKS 1622$-$253& J1625.7$-$2526 & 0.786& \cite{1994MNRAS.269..998D} & Q& G,R \\ 
1622$-$297 & PKS 1622$-$29& J1626.1$-$2948 & 0.815& \cite{1994AAS..105..211S} & Q& R \\ 
1633+382 & 4C +38.41& J1635.2+3810 & 1.813& \cite{2012ApJ...748...49S} & Q& G,R \\ 
1637+574 & OS 562&\n & 0.751& \cite{1996ApJS..104...37M} & Q& R \\ 
1637+826 & NGC 6251& J1629.4+8236 & 0.024& \cite{2003AJ....126.2268W} & G& L \\ 
1638+398 & NRAO 512& J1640.7+3945 & 1.666& \cite{1989AAS...80..103S} & Q& R \\ 
1641+399 & 3C 345& J1642.9+3949 & 0.593& \cite{1996ApJS..104...37M} & Q& G,R \\ 
1642+690 & 4C +69.21&\n & 0.751& \cite{1986AJ.....91..494L} & Q& R \\ 
1652+398\tablenotemark{a} & Mrk 501& J1653.9+3945 & 0.0337& \cite{1993AAS...98..393S} & B& G,L \\ 
1655+077 & PKS 1655+077&\n & 0.621& \cite{1986MNRAS.218..331W} & Q& R \\ 
1700+685 & TXS 1700+685& J1700.2+6831 & 0.301& \cite{1997MNRAS.290..380H} & Q& G,L \\ 
1717+178 & OT 129& J1719.3+1744 & 0.137& \cite{2005ApJ...626...95S} & B& G,L \\ 
1722+119\tablenotemark{a} & 1H 1720+117& J1725.0+1151 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1726+455 & S4 1726+45& J1727.1+4531 & 0.717& \cite{1997MNRAS.290..380H} & Q& R \\ 
1730$-$130 & NRAO 530& J1733.1$-$1307 & 0.902& \cite{1984PASP...96..539J} & Q& G,R \\ 
1732+389 & OT 355& J1734.3+3858 & 0.975& \cite{2012ApJ...748...49S} & Q& G \\ 
1739+522 & 4C +51.37& J1740.2+5212 & 1.379& \cite{1984MNRAS.211..105W} & Q& G,R \\ 
1741$-$038 & PKS 1741$-$03&\n & 1.054& \cite{1988ApJ...327..561W} & Q& R \\ 
1749+096 & 4C +09.57& J1751.5+0938 & 0.322& \cite{1988AA...191L..16S} & B& G,R \\ 
1751+288 & B2 1751+28&\n & 1.118& \cite{2008ApJS..175...97H} & Q& R \\ 
1758+388 & B3 1758+388B&\n & 2.092& \cite{1994AAS..103..349S} & Q& R \\ 
1800+440 & S4 1800+44& J1801.7+4405 & 0.663& \cite{1982MNRAS.200..191W} & Q& R \\ 
1803+784 & S5 1803+784& J1800.5+7829 & 0.6797& \cite{1996ApJS..107..541L} & B& G,R \\ 
1807+698 & 3C 371& J1806.7+6948 & 0.051& \cite{1992AAS...96..389d} & B& G,R,L \\ 
1823+568 & 4C +56.27& J1824.0+5650 & 0.664& \cite{1986AJ.....91..494L} & B& G,R \\ 
1828+487 & 3C 380& J1829.7+4846 & 0.692& \cite{1996ApJS..107..541L} & Q& R \\ 
1842+681 & GB6 J1842+6809&\n & 0.472& \cite{1994AJ....108..395X} & Q& R \\ 
1845+797 & 3C 390.3&\n & 0.0555& \cite{1994ApJS...90....1E} & G& L \\ 
1846+322 & B2 1846+32A& J1848.5+3216 & 0.80& \cite{2012ApJ...748...49S} & Q& G \\ 
1849+670 & S4 1849+67& J1849.4+6706 & 0.657& \cite{1993AAS..100..395S} & Q& G,R \\ 
1902+556 & TXS 1902+556& J1903.3+5539 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
1908$-$201 & PKS B1908$-$201& J1911.1$-$2005 & 1.119& \cite{2003AJ....125..572H} & Q& G,R \\ 
1920$-$211 & OV -235& J1923.5$-$2105 & 0.874& \cite{2003AJ....125..572H} & Q& G,R \\ 
1921$-$293 & PKS B1921$-$293& J1924.8$-$2912 & 0.3526& \cite{2009MNRAS.399..683J} & Q& R \\ 
1923+210 & PKS B1923+210&\n & \n& \n & B& R \\ 
1928+738 & 4C +73.18&\n & 0.302& \cite{1986AJ.....91..494L} & Q& R \\ 
1936$-$155 & PKS 1936$-$15&\n & 1.657& \cite{1984ApJ...286..498J} & Q& R \\ 
1951$-$115 & TXS 1951$-$115& J1954.6$-$1122 & 0.683& \cite{2012ApJ...748...49S} & Q& G \\ 
1957+405 & Cygnus A&\n & 0.0561& \cite{1997ApJ...488L..15O} & G& R,L \\ 
1958$-$179 & PKS 1958$-$179& J2000.8$-$1751 & 0.652& \cite{1975MNRAS.173p..87B} & Q& G,R \\ 
1959+650\tablenotemark{a} & 1ES 1959+650& J2000.0+6509 & 0.047& \cite{1993ApJ...412..541S} & B& G,L \\ 
2005+403 & TXS 2005+403&\n & 1.736& \cite{1976MNRAS.177p..43B} & Q& R \\ 
2007+777 & S5 2007+77& J2004.5+7754 & 0.342& \cite{1989AAS...80..103S} & B& R \\ 
2008$-$159 & PKS 2008$-$159&\n & 1.180& \cite{1979ApJ...232..400P} & Q& R \\ 
2013+370 & MG2 J201534+3710& J2015.6+3709 & 0.859& \cite{2013ApJ...764..135S} & Q& R \\ 
2021+317 & 4C +31.56&\n & 0.356& \n & U& R \\ 
2021+614 & OW 637&\n & 0.227& \cite{1984ApJ...279..112B} & G& R \\ 
2022$-$077 & PKS 2023$-$07& J2025.6$-$0736 & 1.388& \cite{1997MNRAS.284...85D} & Q& G \\ 
2023+335 & B2 2023+33& J2025.1+3341 & 0.219& \cite{2003ApJ...590..109S} & Q& R \\ 
2029+121 & PKS 2029+121& J2031.7+1223 & 1.213& \cite{2012ApJ...748...49S} & Q& R \\ 
2037+511 & 3C 418&\n & 1.686& \cite{1985PASP...97..932S} & Q& R \\ 
2121+053 & PKS 2121+053&\n & 1.941& \cite{1991ApJ...382..433S} & Q& R \\ 
2128$-$123 & PKS 2128$-$12&\n & 0.501& \cite{1968ApJ...154L.101S} & Q& R \\ 
2131$-$021 & 4C $-$02.81& J2133.8$-$0154 & 1.284& \cite{1997MNRAS.284...85D} & Q& R \\ 
2134+004 & PKS 2134+004&\n & 1.932& \cite{1994ApJ...436..678O} & Q& R \\ 
2136+141 & OX 161&\n & 2.427& \cite{1974ApJ...190..271W} & Q& R \\ 
2141+175 & OX 169& J2143.5+1743 & 0.2107& \cite{2009ApJS..184..398H} & Q& G,L \\ 
2144+092 & PKS 2144+092& J2147.3+0930 & 1.113& \cite{1988ApJ...327..561W} & Q& G \\ 
2145+067 & 4C +06.69& J2148.2+0659 & 0.999& \cite{1991ApJ...382..433S} & Q& R \\ 
2155$-$152 & PKS 2155$-$152& J2157.9$-$1501 & 0.672& \cite{1988ApJ...327..561W} & Q& R \\ 
2200+420\tablenotemark{a} & BL Lac& J2202.8+4216 & 0.0686& \cite{1995ApJ...452L...5V} & B& G,R,L \\ 
2201+171 & PKS 2201+171& J2203.4+1726 & 1.076& \cite{1977ApJ...215..427S} & Q& G,R \\ 
2201+315 & 4C +31.63&\n & 0.2947& \cite{1996ApJS..104...37M} & Q& R \\ 
2209+236 & PKS 2209+236& J2211.9+2355 & 1.125& \cite{2003ApJ...590..109S} & Q& R \\ 
2216$-$038 & PKS 2216$-$03&\n & 0.901& \cite{1967ApJ...147..837L} & Q& R \\ 
2223+210 & DA 580&\n & 1.959& \cite{1994ApJS...93....1A} & Q& R \\ 
2223$-$052 & 3C 446& J2225.6$-$0454 & 1.404& \cite{1983MNRAS.205..793W} & Q& G,R \\ 
2227$-$088 & PHL 5225& J2229.7$-$0832 & 1.5595& \cite{2004AJ....128..502A} & Q& G,R \\ 
2230+114 & CTA 102& J2232.4+1143 & 1.037& \cite{1994ApJS...93..125F} & Q& G,R \\ 
2233$-$148 & OY -156& J2236.5$-$1431 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
2234+282 & CTD 135& J2236.4+2828 & 0.790& \cite{2012ApJ...748...49S} & B& G,R \\ 
2241+200 & RGB J2243+203& J2243.9+2021 & \n& \cite{2013ApJ...764..135S} & B& G \\ 
2243$-$123 & PKS 2243$-$123&\n & 0.632& \cite{1975MNRAS.173p..87B} & Q& R \\ 
2247$-$283 & PMN J2250$-$2806& J2250.8$-$2808 & 0.525& \cite{2012ApJ...748...49S} & Q& G \\ 
2251+158 & 3C 454.3& J2253.9+1609 & 0.859& \cite{1991MNRAS.250..414J} & Q& G,R \\ 
2254+074 & PKS 2254+074&\n & 0.190& \cite{1988AA...191L..16S} & B& L \\ 
2255$-$282 & PKS 2255$-$282& J2258.0$-$2759 & 0.927& \cite{2009MNRAS.399..683J} & Q& R \\ 
2325+093 & OZ 042& J2327.5+0940 & 1.841& \cite{2012ApJ...748...49S} & Q& G,R \\ 
2328$-$220 & PMN J2331$-$2148& J2330.9$-$2144 & 0.563& \cite{2012ApJ...748...49S} & Q& G \\ 
2331+073 & TXS 2331+073& J2334.3+0734 & 0.401& \cite{2005ApJ...626...95S} & Q& R \\ 
2344+514\tablenotemark{a} & 1ES 2344+514& J2347.0+5142 & 0.044& \cite{1996ApJS..104..251P} & B& L \\ 
2345$-$167 & PKS 2345$-$16& J2347.9$-$1629 & 0.576& \cite{1993MNRAS.263..999T} & Q& R \\ 
2351+456 & 4C +45.51&\n & 1.986& \cite{1996ApJS..107..541L} & Q& R \\ 
\enddata 

\tablenotetext{a}{Known TeV emitter (http://tevcat.uchicago.edu).}
\tablecomments{Columns are as follows: 
(1) B1950 name, 
(2) other name,
(3) 2FGL catalog name,
(4) redshift,
(5) literature reference for redshift and optical classification,
(6) optical classification, where B = BL Lac, Q=Quasar, G = Radio galaxy, N = Narrow Line Seyfert 1, and U = Unidentified,
(7) Sample membership, where G=1FM $\gamma$-ray selected sample, R = MOJAVE 1.5 Jy sample, L = low-luminosity sample.
}

\end{deluxetable} 

